FreeRide: Harvesting Bubbles in Pipeline Parallelism

The occurrence of bubbles in pipeline parallelism is an inherent limitation that can account for more than 40% of the large language model (LLM) training time and is one of the main reasons for the underutilization of GPU resources in LLM training. Harvesting these bubbles for GPU side tasks can increase resource utilization and reduce training costs but comes with challenges. First, because bubbles are discontinuous with various shapes, programming side tasks becomes difficult while requiring excessive engineering effort. Second, a side task can compete with pipeline training for GPU resources and incur significant overhead. To address these challenges, we propose FreeRide, a system designed to harvest bubbles in pipeline parallelism for side tasks. FreeRide provides programmers with interfaces to implement side tasks easily, manages bubbles and side tasks during pipeline training, and controls access to GPU resources by side tasks to reduce overhead. We demonstrate that FreeRide achieves 7.8% average cost savings with a negligible overhead of about 1% in training LLMs while serving model training, graph analytics, and image processing side tasks.

==> a_new_side_task.tex <==
\subsection{Comparison of GPU Workload Throughput}\label{sec:new_side_task}

Table~\ref{tab:tput} compares the throughput of GPU workloads in Table~\ref{tab:e2e} running on bubbles using the iterative interface of \bb{} (the Iterative column), on Server-II as introduced in Section~\ref{sec:meth} (the Server-II column) and on an 8-core CPU server (the CPU server column).
The throughput is measured by iterations per second.
For ResNet18, ResNet50, and VGG19 GPU workloads, one iteration corresponds to one batch of training data.
For PageRank and Graph SGD, in each iteration, the graph algorithm runs over the input graph for one step.
For image processing workload, one iteration processes one image.

This comparison shows that although side tasks run only during bubbles, they still achieve higher throughput compared to running on a standalone lower-tier GPU server or an 8-core CPU server.
This demonstrates \bb{}'s effectiveness in harvesting the bubbles in pipeline parallel training.
By introducing very little overhead to pipeline parallel training, \bb{} harvests GPU resources that are 1.05x to 2.82x of a standalone lower-tier GPU.

\begin{table}
\caption{Throughput of GPU workloads on different platforms measured in iterations per second.}
\label{tab:tput}
\begin{tabular}{cccc}
\toprule
Workload  & Iterative & Server-II & CPU server  \\ \midrule
ResNet18  & 1586.6             & 998.7     & 26.5 \\
ResNet50  & 533.1              & 393.4     & 9.1 \\
VGG19     & 170.7              & 161.8     & 3.0 \\
PageRank  & 333.9              & 126.3     & 11.1      \\
Graph SGD & 4.2                & 1.5       & 0.6       \\
Image     & 12.2               & 7.8       & 1.6         \\ \bottomrule
\end{tabular}
\end{table}



